LLMorpheus: Mutation Testing using Large Language Models

In mutation testing, the quality of a test suite is evaluated by introducing faults into a program and determining whether the program's tests detect them. Most existing approaches for mutation testing involve the application of a fixed set of mutation operators, e.g., replacing a "+" with a "-", or removing a function's body. However, certain types of real-world bugs cannot easily be simulated by such approaches, limiting their effectiveness. This paper presents a technique for mutation testing where placeholders are introduced at designated locations in a program's source code and where a Large Language Model (LLM) is prompted to ask what they could be replaced with. The technique is implemented in LLMorpheus, a mutation testing tool for JavaScript, and evaluated on 13 subject packages, considering several variations on the prompting strategy, and using several LLMs. We find LLMorpheus to be capable of producing mutants that resemble existing bugs that cannot be produced by StrykerJS, a state-of-the-art mutation testing tool. Moreover, we report on the running time, cost, and number of mutants produced by LLMorpheus, demonstrating its practicality.

==> figures/fig-ComplexJSExample.tex <==
\begin{figure*}
\centering

\begin{tabular}{c}
\includegraphics[width=0.75\textwidth]{figures/ComplexJSCommit.png}
\\
{\bf (a)}
\\[3mm]
\includegraphics[width=0.55\textwidth]{figures/ComplexJSMutant1.png}
\\
{\bf (b)}
\\[3mm]
\includegraphics[width=0.55\textwidth]{figures/ComplexJSMutant2.png}
\\
{\bf (c)}
\end{tabular}
\caption{
  (a) Fix for a bug in \code{Complex.js}.
  (b) A mutation suggested by \ToolName elsewhere in the same file that involves replacing a 
      binary expression with one of its subexpressions.
  (c) A mutation suggested by \ToolName elsewhere in the same file that involves replacing a 
      simple expression with a binary expression. 
}
\label{fig:ComplexJSExample}
\end{figure*}

==> figures/table-codellama13-full-0.0-variability.tex <==
% This table was generated -- DO NOT EDIT
\begin{table}
\centering
{\footnotesize
\begin{tabular}{l|r|r|r|r}
{\bf application}  & {\bf \#min} &  {\bf \#max} &  {\bf \#distinct} & {\bf \#common}\\
\hline
Complex.js & 955 & 955 & 955 & 955 (100.00\%) \\ 
countries-and-timezones & 207 & 207 & 207 & 207 (100.00\%) \\ 
crawler-url-parser & 257 & 257 & 257 & 257 (100.00\%) \\ 
delta & 712 & 712 & 713 & 711 (99.72\%) \\ 
image-downloader & 77 & 77 & 77 & 77 (100.00\%) \\ 
node-dirty & 245 & 245 & 245 & 245 (100.00\%) \\ 
node-geo-point & 305 & 305 & 305 & 305 (100.00\%) \\ 
node-jsonfile & 137 & 138 & 138 & 137 (99.28\%) \\ 
plural & 200 & 208 & 394 & 14 (3.55\%) \\ 
pull-stream & 668 & 669 & 671 & 666 (99.25\%) \\ 
q & 1713 & 1715 & 1725 & 1702 (98.67\%) \\ 
spacl-core & 195 & 195 & 197 & 193 (97.97\%) \\ 
zip-a-folder & 87 & 87 & 87 & 87 (100.00\%) \\ 
\end{tabular}
}
\caption{
  Variability of the mutants generated in 5 runs of \ToolName at temperature 0 using the \CodeLlamaThirteen LLM. 
  The columns of the table show, from left to right:  
    (i) the minimum number of mutants observed in any of the runs,
    (ii) the maximum number of mutants observed in any of the runs,
    (iii) the total number of distinct mutants observed in all runs, and
    (iv) the number (percentage) of mutants are observed in all runs.
}
\label{table:CodeLlama13Variability}
\end{table}

==> figures/table-codellama13-full-0.0.tex <==
 \begin{table*}
 \centering
 {\scriptsize
 \begin{tabular}{l||r|r|r|r|r|r||r|r||r|r|r}
   {\bf application}                & {\bf \#prompts}   & {\bf \#mutants} & {\bf \#killed} & {\bf \#survived} & {\bf \#timeout} & \multicolumn{1}{|c||}{\bf mut.}   & \multicolumn{2}{|c||}{\bf time (sec)} & \multicolumn{3}{|c}{\bf \#tokens}\\
                                    &                   &                 &                &                  &                 & \multicolumn{1}{|c||}{\bf score}    & \ToolName & {\it StrykerJS}  & {\bf prompt} & {\bf compl.} & {\bf total}\\
   \hline
   \textit{Complex.js} & 490 & 955 & 553 & 401 & 1 & 58.01 & 3,041.69 & 525.25 & 967,508 & 104,246 & 1,071,754 \\ 
   \hline
   \textit{countries-and-timezones} & 106 & 207 & 177 & 30 & 0 & 85.51 & 1,070.79 & 310.80 & 105,828 & 23,971 & 129,799 \\ 
   \hline
   \textit{crawler-url-parser} & 176 & 247 & 129 & 118 & 0 & 52.23 & 1,637.98 & 803.17 & 386,223 & 39,906 & 426,129 \\ 
   \hline
   \textit{delta} & 462 & 712 & 583 & 107 & 22 & 84.97 & 2,993.70 & 3,529.05 & 890,252 & 103,085 & 993,337 \\ 
   \hline
   \textit{image-downloader} & 42 & 77 & 48 & 29 & 0 & 62.34 & 430.56 & 460.64 & 24,655 & 9,339 & 33,994 \\ 
   \hline
   \textit{node-dirty} & 154 & 245 & 142 & 92 & 11 & 62.45 & 1,526.96 & 211.68 & 246,248 & 34,892 & 281,140 \\ 
   \hline
   \textit{node-geo-point} & 140 & 304 & 237 & 67 & 0 & 77.96 & 1,411.04 & 1,000.74 & 316,333 & 30,715 & 347,048 \\ 
   \hline
   \textit{node-jsonfile} & 68 & 138 & 43 & 45 & 50 & 67.39 & 690.65 & 425.39 & 57,516 & 15,398 & 72,914 \\ 
   \hline
   \textit{plural} & 153 & 208 & 154 & 53 & 1 & 74.52 & 1,521.00 & 111.98 & 265,602 & 34,926 & 300,528 \\ 
   \hline
   \textit{pull-stream} & 351 & 669 & 386 & 237 & 46 & 64.57 & 2,489.93 & 1,188.59 & 208,130 & 77,308 & 285,438 \\ 
   \hline
   \textit{q} & 1051 & 1713 & 122 & 1518 & 73 & 11.38 & 5,187.67 & 11,850.22 & 2,127,655 & 231,175 & 2,358,830 \\ 
   \hline
   \textit{spacl-core} & 134 & 185 & 160 & 25 & 0 & 86.49 & 1,350.97 & 616.43 & 162,705 & 30,694 & 193,399 \\ 
   \hline
   \textit{zip-a-folder} & 49 & 87 & 27 & 55 & 5 & 36.78 & 500.51 & 496.32 & 82,457 & 11,494 & 93,951 \\ 
   \hline
   \textit{Total} & 3376 & 5747 & 2761 & 2777 & 209 & - & 23,853.45  & 21,530.26 & 5,841,112 & 747,149 & 6,588,261 \\ 
 \end{tabular}
 }
 \caption{Results obtained with LLMorpheus using the following parameters: 
   model: \textit{codellama-13b-instruct}, 
   temperature: 0, 
   MaxTokens: 250, 
   MaxNrPrompts: 2000, 
   template: \textit{template-full.hb}, 
   systemPrompt: SystemPrompt-MutationTestingExpert.txt, 
   rateLimit: benchmark mode, 
   nrAttempts: 3  
 }
 \label{table:CodeLlama13Full0.0}
\end{table*}
 

==> figures/table-codellama34-full-0.0-variability.tex <==
% table generated using command: "node benchmark/computeVariability.js run312 run314 run315 run316 run317"
\begin{table}
\centering
{\footnotesize
\begin{tabular}{l|r|r|r|r}
{\bf application}  & {\bf \#min} &  {\bf \#max} &  {\bf \#distinct} & {\bf \#common}\\
\hline
Complex.js & 1198 & 1199 & 1217 & 1181 (97.04\%) \\ 
countries-and-timezones & 216 & 217 & 218 & 215 (98.62\%) \\ 
crawler-url-parser & 282 & 285 & 289 & 278 (96.19\%) \\ 
delta & 765 & 768 & 787 & 746 (94.79\%) \\ 
image-downloader & 89 & 90 & 90 & 89 (98.89\%) \\ 
node-dirty & 274 & 275 & 283 & 266 (93.99\%) \\ 
node-geo-point & 302 & 302 & 307 & 297 (96.74\%) \\ 
node-jsonfile & 153 & 154 & 158 & 149 (94.30\%) \\ 
plural & 279 & 281 & 288 & 274 (95.14\%) \\ 
pull-stream & 758 & 760 & 770 & 746 (96.88\%) \\ 
q & 2031 & 2035 & 2053 & 2014 (98.10\%) \\ 
spacl-core & 238 & 239 & 252 & 225 (89.29\%) \\ 
zip-a-folder & 100 & 100 & 102 & 98 (96.08\%) \\ 
\end{tabular}
}
\caption{
  Variability of the mutants generated in 5 runs of \ToolName using the \textit{codellama-34b-instruct} LLM
       at temperature 0.0. The columns of the table show,
  from left to right:  
    (i) the minimum number of mutants observed in any of the runs,
    (ii) the maximum number of mutants observed in any of the runs,
    (iii) the total number of distinct mutants observed in all runs, and
    (iv) the number (percentage) of mutants are observed in all runs.
}
\label{table:variability}
\end{table}

==> figures/table-codellama34-full-0.25.tex <==
\begin{table*}
 \centering
 {\scriptsize
 \begin{tabular}{l||r|r|r|r|r|r||r|r||r|r|r}
   {\bf application}                & {\bf \#prompts}   & {\bf \#mutants} & {\bf \#killed} & {\bf \#survived} & {\bf \#timeout} & \multicolumn{1}{|c||}{\bf mutation}   & \multicolumn{2}{|c||}{\bf time (sec)} & \multicolumn{3}{|c}{\bf \#tokens}\\
                                    &                   &                 &                &                  &                 & \multicolumn{1}{|c||}{\bf score}    & \ToolName & {\it StrykerJS}  & {\bf prompt} & {\bf completion} & {\bf total}\\
   \hline
   \textit{Complex.js} & 490 & 1197 & 730 & 466 & 1 & 61.07 & 3,044.19 & 631.79 & 967,508 & 101,588 & 1,069,096 \\ 
   \hline
   \textit{countries-and-timezones} & 106 & 219 & 181 & 38 & 0 & 82.65 & 1,070.90 & 327.25 & 105,828 & 23,471 & 129,299 \\ 
   \hline
   \textit{crawler-url-parser} & 176 & 260 & 167 & 93 & 0 & 64.23 & 1,646.30 & 818.05 & 386,223 & 39,000 & 425,223 \\ 
   \hline
   \textit{delta} & 462 & 781 & 642 & 111 & 28 & 85.79 & 2,954.37 & 3,844.00 & 890,252 & 99,341 & 989,593 \\ 
   \hline
   \textit{image-downloader} & 42 & 86 & 71 & 15 & 0 & 82.56 & 430.54 & 348.86 & 24,655 & 9,217 & 33,872 \\ 
   \hline
   \textit{node-dirty} & 154 & 279 & 175 & 93 & 11 & 66.67 & 1,532.06 & 232.35 & 246,248 & 32,400 & 278,648 \\ 
   \hline
   \textit{node-geo-point} & 140 & 293 & 225 & 68 & 0 & 76.79 & 1,708.63 & 961.35 & 291,061 & 26,301 & 317,362 \\ 
   \hline
   \textit{node-jsonfile} & 68 & 151 & 52 & 41 & 58 & 72.85 & 740.73 & 502.52 & 57,516 & 14,400 & 71,916 \\ 
   \hline
   \textit{plural} & 153 & 273 & 208 & 63 & 2 & 76.92 & 1,537.89 & 149.38 & 265,602 & 33,182 & 298,784 \\ 
   \hline
   \textit{pull-stream} & 351 & 779 & 452 & 270 & 57 & 65.34 & 2,522.38 & 1,395.14 & 208,130 & 76,091 & 284,221 \\ 
   \hline
   \textit{q} & 1051 & 2050 & 153 & 1813 & 84 & 11.56 & 5,294.80 & 14,085.10 & 2,127,655 & 218,620 & 2,346,275 \\ 
   \hline
   \textit{spacl-core} & 134 & 223 & 187 & 36 & 0 & 83.86 & 1,351.05 & 728.32 & 162,705 & 29,167 & 191,872 \\ 
   \hline
   \textit{zip-a-folder} & 49 & 97 & 24 & 4 & 69 & 95.88 & 500.56 & 1,086.06 & 82,457 & 10,557 & 93,014 \\ 
   \hline
   \textit{Total} & 3376 & 6688 & 3267 & 3111 & 310 & - & 24,334.40  & 25,110.17 & 5,815,840 & 713,335 & 6,529,175 \\ 
 \end{tabular}
 }
 \caption{Results obtained with LLMorpheus using the following parameters: 
   model: \textit{codellama-34b-instruct}, 
   temperature: 0.25, 
   MaxTokens: 250, 
   MaxNrPrompts: 2000, 
   template: \textit{template-full.hb}, 
   systemPrompt: SystemPrompt-MutationTestingExpert.txt, 
   rateLimit: benchmark mode, 
   nrAttempts: 3  
 }
 \label{table:CodeLlama34Full0.25}
\end{table*}

==> figures/table-codellama34-full-0.5.tex <==
\begin{table*}
 \centering
 {\scriptsize
 \begin{tabular}{l||r|r|r|r|r|r||r|r||r|r|r}
   {\bf application}                & {\bf \#prompts}   & {\bf \#mutants} & {\bf \#killed} & {\bf \#survived} & {\bf \#timeout} & \multicolumn{1}{|c||}{\bf mutation}   & \multicolumn{2}{|c||}{\bf time (sec)} & \multicolumn{3}{|c}{\bf \#tokens}\\
                                    &                   &                 &                &                  &                 & \multicolumn{1}{|c||}{\bf score}    & \ToolName & {\it StrykerJS}  & {\bf prompt} & {\bf completion} & {\bf total}\\
   \hline
   \textit{Complex.js} & 490 & 1191 & 739 & 452 & 0 & 62.05 & 3,016.85 & 592.07 & 967,508 & 100,627 & 1,068,135 \\ 
   \hline
   \textit{countries-and-timezones} & 106 & 224 & 194 & 30 & 0 & 86.61 & 1,070.93 & 319.44 & 105,828 & 22,932 & 128,760 \\ 
   \hline
   \textit{crawler-url-parser} & 176 & 298 & 166 & 108 & 24 & 63.76 & 1,668.66 & 1,244.64 & 386,223 & 38,920 & 425,143 \\ 
   \hline
   \textit{delta} & 462 & 769 & 642 & 93 & 34 & 87.91 & 2,980.99 & 3,869.42 & 890,252 & 98,347 & 988,599 \\ 
   \hline
   \textit{image-downloader} & 42 & 89 & 68 & 21 & 0 & 76.40 & 430.55 & 365.90 & 24,655 & 8,925 & 33,580 \\ 
   \hline
   \textit{node-dirty} & 154 & 277 & 158 & 107 & 12 & 61.37 & 1,532.57 & 247.29 & 246,248 & 32,995 & 279,243 \\ 
   \hline
   \textit{node-geo-point} & 140 & 302 & 230 & 72 & 0 & 76.16 & 1,411.06 & 1,006.90 & 316,333 & 29,454 & 345,787 \\ 
   \hline
   \textit{node-jsonfile} & 68 & 153 & 51 & 43 & 59 & 71.90 & 720.71 & 494.61 & 57,516 & 15,051 & 72,567 \\ 
   \hline
   \textit{plural} & 153 & 289 & 219 & 69 & 1 & 76.12 & 1,522.56 & 152.03 & 265,602 & 33,550 & 299,152 \\ 
   \hline
   \textit{pull-stream} & 351 & 796 & 465 & 278 & 53 & 65.08 & 2,506.81 & 1,378.63 & 208,130 & 75,239 & 283,369 \\ 
   \hline
   \textit{q} & 1051 & 2073 & 163 & 1823 & 87 & 12.06 & 5,332.46 & 14,311.02 & 2,127,655 & 217,886 & 2,345,541 \\ 
   \hline
   \textit{spacl-core} & 134 & 250 & 210 & 39 & 1 & 84.40 & 1,351.01 & 850.39 & 162,705 & 28,919 & 191,624 \\ 
   \hline
   \textit{zip-a-folder} & 49 & 87 & 48 & 33 & 6 & 62.07 & 900.98 & 471.62 & 72,362 & 9,438 & 81,800 \\ 
   \hline
   \textit{Total} & 3376 & 6798 & 3353 & 3168 & 277 & - & 24,446.14  & 25,303.96 & 5,831,017 & 712,283 & 6,543,300 \\ 
 \end{tabular}
 }
 \caption{Results obtained with LLMorpheus using the following parameters: 
   model: \textit{codellama-34b-instruct}, 
   temperature: 0.5, 
   MaxTokens: 250, 
   MaxNrPrompts: 2000, 
   template: \textit{template-full.hb}, 
   systemPrompt: SystemPrompt-MutationTestingExpert.txt, 
   rateLimit: benchmark mode, 
   nrAttempts: 3  
 }
  \label{table:CodeLlama34Full0.50}
\end{table*}

==> figures/table-codellama34-full-1.0.tex <==
\begin{table*}
 \centering
 {\scriptsize
 \begin{tabular}{l||r|r|r|r|r|r||r|r||r|r|r}
   {\bf application}                & {\bf \#prompts}   & {\bf \#mutants} & {\bf \#killed} & {\bf \#survived} & {\bf \#timeout} & \multicolumn{1}{|c||}{\bf mutation}   & \multicolumn{2}{|c||}{\bf time (sec)} & \multicolumn{3}{|c}{\bf \#tokens}\\
                                    &                   &                 &                &                  &                 & \multicolumn{1}{|c||}{\bf score}    & \ToolName & {\it StrykerJS}  & {\bf prompt} & {\bf completion} & {\bf total}\\
   \hline
   \textit{Complex.js} & 490 & 1028 & 648 & 379 & 1 & 63.13 & 3,090.47 & 545.31 & 967,508 & 101,516 & 1,069,024 \\ 
   \hline
   \textit{countries-and-timezones} & 106 & 186 & 156 & 30 & 0 & 83.87 & 1,070.88 & 268.04 & 105,828 & 23,041 & 128,869 \\ 
   \hline
   \textit{crawler-url-parser} & 176 & 278 & 202 & 76 & 0 & 72.66 & 1,786.52 & 902.86 & 377,644 & 36,825 & 414,469 \\ 
   \hline
   \textit{delta} & 462 & 698 & 583 & 83 & 32 & 88.11 & 3,134.68 & 3,531.25 & 877,266 & 93,814 & 971,080 \\ 
   \hline
   \textit{image-downloader} & 42 & 75 & 53 & 22 & 0 & 70.67 & 430.55 & 457.54 & 24,655 & 9,002 & 33,657 \\ 
   \hline
   \textit{node-dirty} & 154 & 246 & 150 & 84 & 12 & 65.85 & 1,526.84 & 215.86 & 246,248 & 32,721 & 278,969 \\ 
   \hline
   \textit{node-geo-point} & 140 & 273 & 213 & 60 & 0 & 78.02 & 1,411.05 & 897.39 & 316,333 & 29,494 & 345,827 \\ 
   \hline
   \textit{node-jsonfile} & 68 & 132 & 50 & 22 & 60 & 83.33 & 710.73 & 477.34 & 57,516 & 14,447 & 71,963 \\ 
   \hline
   \textit{plural} & 153 & 299 & 229 & 69 & 1 & 76.92 & 1,533.27 & 157.43 & 265,602 & 31,993 & 297,595 \\ 
   \hline
   \textit{pull-stream} & 351 & 743 & 461 & 235 & 47 & 68.37 & 2,504.20 & 1,268.62 & 208,130 & 73,625 & 281,755 \\ 
   \hline
   \textit{q} & 1051 & 1899 & 147 & 1671 & 81 & 12.01 & 5,355.10 & 13,120.09 & 2,127,655 & 213,824 & 2,341,479 \\ 
   \hline
   \textit{spacl-core} & 134 & 218 & 180 & 38 & 0 & 82.57 & 1,351.04 & 679.82 & 162,705 & 28,574 & 191,279 \\ 
   \hline
   \textit{zip-a-folder} & 49 & 96 & 54 & 38 & 4 & 60.42 & 500.58 & 493.11 & 82,457 & 10,747 & 93,204 \\ 
   \hline
   \textit{Total} & 3376 & 6171 & 3126 & 2807 & 238 & - & 24,405.91  & 23,014.66 & 5,819,547 & 699,623 & 6,519,170 \\ 
 \end{tabular}
 }
 \caption{Results obtained with LLMorpheus using the following parameters: 
   model: \textit{codellama-34b-instruct}, 
   temperature: 1, 
   MaxTokens: 250, 
   MaxNrPrompts: 2000, 
   template: \textit{template-full.hb}, 
   systemPrompt: SystemPrompt-MutationTestingExpert.txt, 
   rateLimit: benchmark mode, 
   nrAttempts: 3  
 }
   \label{table:CodeLlama34Full1.0}
\end{table*}

==> figures/table-strykermutants.tex <==
\begin{table}
 \centering
 {\scriptsize
 \begin{tabular}{l||r|r|r|r|r|r}
   {\bf application} & \Total & \Killed & \Survived & \Timeout & \MutScore & \Time\\
   \hline
   \textit{Complex.js} & 1302 & 763 & 539 & 0 & 58.60 & 687.01 \\ 
   \hline
   \textit{countries-and-timezones} & 140 & 134 & 6 & 0 & 95.71 & 205.88 \\ 
   \hline
   \textit{crawler-url-parser} & 226 & 143 & 83 & 0 & 63.27 & 739.58 \\ 
   \hline
   \textit{delta} & 834 & 686 & 88 & 60 & 89.45 & 4,200.75 \\ 
   \hline
   \textit{image-downloader} & 43 & 28 & 11 & 4 & 74.42 & 299.72 \\ 
   \hline
   \textit{node-dirty} & 160 & 78 & 56 & 26 & 65.00 & 267.33 \\ 
   \hline
   \textit{node-geo-point} & 158 & 98 & 60 & 0 & 62.03 & 502.91 \\ 
   \hline
   \textit{node-jsonfile} & 61 & 31 & 5 & 25 & 91.80 & 220.17 \\ 
   \hline
   \textit{plural} & 180 & 143 & 37 & 0 & 79.44 & 92.90 \\ 
   \hline
   \textit{pull-stream} & 474 & 318 & 116 & 40 & 75.53 & 834.18 \\ 
   \hline
   \textit{q} & 1058 & 68 & 927 & 63 & 12.38 & 7,516.19 \\ 
   \hline
   \textit{spacl-core} & 259 & 239 & 20 & 0 & 92.28 & 813.55 \\ 
   \hline
   \textit{zip-a-folder} & 74 & 38 & 8 & 28 & 89.19 & 604.29 \\ 
   \hline
   \textit{Total} & 4969 & 2767 & 1956 & 246 & - & 16,984.46 \\ 
 \end{tabular}
 }
 \caption{Results of applying the standard mutation operators of \StrykerJS.
 }
 \label{table:StrykerMutants}
\end{table}
